SoK: Safer Digital-Safety Research Involving At-Risk Users

Research involving at-risk users -- that is, users who are more likely to experience a digital attack or to be disproportionately affected when harm from such an attack occurs -- can pose significant safety challenges to both users and researchers. Nevertheless, pursuing research in computer security and privacy is crucial to understanding how to meet the digital-safety needs of at-risk users and to design safer technology for all. To standardize and bolster safer research involving such users, we offer an analysis of 196 academic works to elicit 14 research risks and 36 safety practices used by a growing community of researchers. We pair this inconsistent set of reported safety practices with oral histories from 12 domain experts to contribute scaffolded and consolidated pragmatic guidance that researchers can use to plan, execute, and share safer digital-safety research involving at-risk users. We conclude by suggesting areas for future research regarding the reporting, study, and funding of at-risk user research

==> 07-conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

\noindent Despite a growing body of research in S\&P and HCI that is drawing attention to the digital-safety needs and experiences of at-risk users, there has been little consensus on how to conduct this research safely.
We conducted an analysis of \paperNo papers on digital safety and at-risk users, and identified \iriskNo explicitly articulated risks addressed by the authors and \isafetyNo safety practices they reported using to mitigate the risks.
We paired this analysis with oral histories from 12 experts to contribute \strategyNo strategies that scaffold and consolidate pragmatic guidance researchers can use to plan, execute, and share safer at-risk research. This systematization provides foundational guidance for safer digital-safety research involving at-risk users. We also hope our strategies will help the community work toward more consistent reporting of safety strategies employed in at-risk research.


==> figs-tabs/lit-comparison.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[]
\tiny
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}l|c|c|c|c|@{}}
% \cmidrule(l){2-5}
 & At-risk group focus & Multiple at-risk groups & Research harms & Literature review \\ \midrule
Bhalerao et al. \cite{bhalerao_ethical_2022} & $\times$ & $\times$ & $\times$ &   \\
Distler et al. \cite{distler_systematic_2021} &  &  & $\times$ & $\times$ \\
Sannon et al. \cite{sannon_privacy_2022}   &   & $\times$ & $\times$ & $\times$ \\
Slupska et al. \cite{slupska2021participatory} & $\times$ &   &   &  \\
Thomas et al. \cite{thomas_sok_2021} &  & $\times$ &  &  $\times$ \\
Warford et al. \cite{warford2022atrisk} & $\times$ & $\times$ &   & $\times$ \\ \bottomrule
\end{tabular}%
}
\caption{\footnotesize{Table comparing the characteristics of related S\&P work on digital safety concerns with at-risk groups. $\times$ signifies that work addresses this factor; blank signifies it does not.}}
\label{tab:digital-comparison}
\end{table}

==> figs-tabs/methods.tex <==
\begin{table*}[]
\tiny
\resizebox{\textwidth}{!}{%
\begin{tabular}{lclclc}
\textbf{Method Category} & \textbf{Count} &  &  &  &  \\ \hline
\textbf{Interview} & 89 & \textbf{Creativity-Based Approaches} & 25 & \textbf{Tool Evaluation} & 33 \\ \cline{1-1} \cline{3-3} \cline{5-5}
Semi-Structured Interview & 76 & Co-Design Sessions & 3 & Testing Design Mockups & 4 \\
In-Depth Interview & 4 & Illustration & 5 & Tool Evaluation & 23 \\
Structured Interview & 6 & Card Sorting Exercise & 2 & Speak-Aloud Walkthroughs & 1 \\
Narrative Interview & 2 & Design Workshop & 14 & Artefact Analysis & 1 \\
\textbf{Survey} & 53 & \textbf{Measurement Studies} & 25 & Personal device examination & 1 \\ \cline{1-1} \cline{3-3}
Online Survey & 30 & Social Media Scrape & 13 & Log Analysis & 3 \\
Pre-Deployment survey & 4 & Web scrape & 3 & \textbf{Observation-Based} & 19 \\ \cline{5-5}
Post-Deployment Survey & 10 & Measurement Pipeline & 3 & Ethnography & 7 \\
Demographic survey & 9 & App Audit & 6 & Online Ethnography & 2 \\
\textbf{Group Discussion} & 20 & \textbf{Document-Based} & 8 & Field Observations & 10 \\ \cline{1-1} \cline{3-3}
Focus Groups & 17 & Diary Study & 4 & \textbf{Critical Analysis} & 5 \\ \cline{5-5}
Focused Group Discussions & 3 & Document Analysis & 4 & Case study-based & 5
\end{tabular}%
}
\label{tab:method-breakdown}
\caption{Data collection approaches used in digital-safety research with and about at-risk groups. We note that individual papers may use more than one method.}
\end{table*}
